Testing predictions of representation cost theory with CNNs

It is widely acknowledged that trained convolutional neural networks (CNNs) have different levels of sensitivity to signals of different frequency. In particular, a number of empirical studies have documented CNNs sensitivity to low-frequency signals. In this work we show with theory and experiments that this observed sensitivity is a consequence of the frequency distribution of natural images, which is known to have most of its power concentrated in low-to-mid frequencies. Our theoretical analysis relies on representations of the layers of a CNN in frequency space, an idea that has previously been used to accelerate computations and study implicit bias of network training algorithms, but to the best of our knowledge has not been applied in the domain of model robustness.

==> model_details.tex <==
\begin{footnotesize}
    \begin{longtable}[]{@{}
       >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.2000}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.2000}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.2000}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.2000}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.2000}}@{}}
     \toprule()
     \begin{minipage}[b]{\linewidth}\raggedright
     arch. family
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     depth
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     batch size
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     initial lr
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     decay
     \end{minipage} \\
     \midrule()
     \endhead
     Conv Actually & 4 & 1024 & \(10^{-4}\) &
     \texttt{10**linspace(-5,\ -1,\ 4)} \\
     Myrtle CNN & N/A & 512 & \(10^{-2}\) &
     \texttt{10**linspace(-5,\ -2,\ 10)} \\
     CIFAR VGG & 11 & 256 & \(10^{-2}\) &
     \texttt{10**linspace(-5,\ -2,\ 10)} \\
     ImageNette VGG & 11 & 256 & \(1.250 \times 10^{-3}\) &
     \texttt{10**linspace(-5,\ -2,\ 3)} \\
     ResNet & 9 & 512 & \(10^{-1}\) & \texttt{10**linspace(-5,\ -2,\ 10)} \\
     \bottomrule()
     \caption{Hyperparameters of CNNs of variable decay used in the experiments of
     \cref{sec:freq-sens-decay}. In all cases, the maximum number of epochs was \(500\).}\label{tab:hparam-decay}
     \end{longtable}
 \end{footnotesize}
 
 \begin{footnotesize}
    \begin{longtable}[]{@{}
       >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.2000}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.2000}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.2000}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.2000}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.2000}}@{}}
     \toprule()
     \begin{minipage}[b]{\linewidth}\raggedright
     arch. family
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     depth
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     batch size
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     initial lr
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     max epochs
     \end{minipage} \\
     \midrule()
     \endhead
     Conv Actually & 1,2,4,8 & 1024 & \(10^{-4}\) & 500 \\
     CIFAR VGG & 11, 13, 16, 19 & 256 & \(10^{-2}\) & 500 \\
     ImageNette VGG & 11, 13, 16 , 19 & 256 & \(1.250 \times 10^{-3}\) &
     500 \\
     ResNet & 9, 20, 56 & 512 & \(10^{-1}\) & 200 \\
     \bottomrule()
     \caption{Hyperparameters of CNNs of variable depth used in the experiments of
     \cref{sec:freq-sens-depth}.}\label{tab:hparam-depth}
     \end{longtable}
 \end{footnotesize}
 
  \hypertarget{model-validation-accuracies}{%
 \subsubsection{Model validation
 accuracies}\label{model-validation-accuracies}}
 
 
 \begin{longtable}[]{@{}
   >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.2174}}
   >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.1957}}
   >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.1957}}
   >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.1957}}
   >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.1957}}@{}}
 \toprule()
 \begin{minipage}[b]{\linewidth}\raggedright
 \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
 1e-05
 \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
 0.0002154
 \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
 0.004642
 \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
 0.1
 \end{minipage} \\
 \midrule()
 \endhead
 natural & 0.628 \(+-\) 0.002 & 0.626 \(+-\) 0.011 & 0.631 \(+-\) 0.006 &
 0.641 \(+-\) 0.009 \\
 hpf & 0.513 \(+-\) 0.028 & 0.518 \(+-\) 0.015 & 0.534
 \(+-\) 0.033 & 0.484 \(+-\) 0.008 \\
 \bottomrule()\caption{Validation accuracies for ConvActually, variable
 decay}
 \end{longtable}
 
 \begin{tiny}
    \begin{longtable}[]{@{}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.0926}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.0833}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.0833}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.1204}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.0833}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.0833}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.1204}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.0833}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.0833}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.0833}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.0833}}@{}}
     \toprule()
     \begin{minipage}[b]{\linewidth}\raggedright
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     1e-05
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     2.154e-05
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     4.642e-05
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     0.0001
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     0.0002154
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     0.0004642
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     0.001
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     0.002154
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     0.004642
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     0.01
     \end{minipage} \\
     \midrule()
     \endhead
     natural & 0.866 \(+-\) 0.003 & 0.864 \(+-\) 0.002 & 0.866 \(+-\) 0.003 &
     0.863 \(+-\) 0.003 & 0.866 \(+-\) 0.003 & 0.868 \(+-\) 0.001 & 0.867
     \(+-\) 0.003 & 0.869 \(+-\) 0.001 & 0.868 \(+-\) 0.002 & 0.836 \(+-\)
     0.003 \\
     hpf & 0.791 \(+-\) 0.004 & 0.795 \(+-\) 0.004 & 0.794
     \(+-\) 0.003 & 0.796 \(+-\) 0.002 & 0.795 \(+-\) 0.002 & 0.797 \(+-\)
     0.003 & 0.797 \(+-\) 0.004 & 0.793 \(+-\) 0.004 & 0.782 \(+-\) 0.006 &
     0.747 \(+-\) 0.002 \\
     \bottomrule()\caption{Validation accuracies for Myrtle CNN, variable
     decay}
     \end{longtable}
 \end{tiny}
 
 \begin{tiny}
    \begin{longtable}[]{@{}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.0926}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.0833}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.0833}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.1204}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.0833}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.0833}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.1204}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.0833}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.0833}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.0833}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.0833}}@{}}
     \toprule()
     \begin{minipage}[b]{\linewidth}\raggedright
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     1e-05
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     2.154e-05
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     4.642e-05
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     0.0001
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     0.0002154
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     0.0004642
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     0.001
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     0.002154
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     0.004642
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     0.01
     \end{minipage} \\
     \midrule()
     \endhead
     natural & 0.920 \(+-\) 0.002 & 0.920 \(+-\) 0.001 & 0.920 \(+-\) 0.002 &
     0.923 \(+-\) 0.001 & 0.925 \(+-\) 0.002 & 0.929 \(+-\) 0.001 & 0.935
     \(+-\) 0.002 & 0.936 \(+-\) 0.001 & 0.928 \(+-\) 0.002 & 0.912 \(+-\)
     0.004 \\
     hpf & 0.850 \(+-\) 0.006 & 0.853 \(+-\) 0.001 & 0.853
     \(+-\) 0.001 & 0.849 \(+-\) 0.003 & 0.849 \(+-\) 0.003 & 0.861 \(+-\)
     0.004 & 0.862 \(+-\) 0.004 & 0.864 \(+-\) 0.006 & 0.862 \(+-\) 0.004 &
     0.844 \(+-\) 0.007 \\
     \bottomrule()\caption{Validation accuracies for ResNet, variable decay}
     \end{longtable}
 \end{tiny}
 
 \begin{tiny}
    \begin{longtable}[]{@{}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.0926}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.0833}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.0833}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.1204}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.0833}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.0833}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.1204}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.0833}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.0833}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.0833}}
       >{\raggedright\arraybackslash}p{(\columnwidth - 20\tabcolsep) * \real{0.0833}}@{}}
     \toprule()
     \begin{minipage}[b]{\linewidth}\raggedright
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     1e-05
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     2.154e-05
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     4.642e-05
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     0.0001
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     0.0002154
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     0.0004642
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     0.001
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     0.002154
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     0.004642
     \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
     0.01
     \end{minipage} \\
     \midrule()
     \endhead
     natural & 0.872 \(+-\) 0.003 & 0.871 \(+-\) 0.002 & 0.874 \(+-\) 0.004 &
     0.874 \(+-\) 0.002 & 0.875 \(+-\) 0.002 & 0.876 \(+-\) 0.002 & 0.883
     \(+-\) 0.002 & 0.885 \(+-\) 0.001 & 0.881 \(+-\) 0.002 & 0.836 \(+-\)
     0.013 \\
     hpf & 0.795 \(+-\) 0.002 & 0.793 \(+-\) 0.003 & 0.794
     \(+-\) 0.002 & 0.798 \(+-\) 0.004 & 0.799 \(+-\) 0.003 & 0.801 \(+-\)
     0.003 & 0.805 \(+-\) 0.001 & 0.809 \(+-\) 0.002 & 0.789 \(+-\) 0.008 &
     0.169 \(+-\) 0.123 \\
     \bottomrule()\caption{Validation accuracies for VGG (CIFAR), variable
     decay}
     \end{longtable}
 \end{tiny}
 
 \begin{longtable}[]{@{}
   >{\raggedright\arraybackslash}p{(\columnwidth - 6\tabcolsep) * \real{0.2703}}
   >{\raggedright\arraybackslash}p{(\columnwidth - 6\tabcolsep) * \real{0.2432}}
   >{\raggedright\arraybackslash}p{(\columnwidth - 6\tabcolsep) * \real{0.2432}}
   >{\raggedright\arraybackslash}p{(\columnwidth - 6\tabcolsep) * \real{0.2432}}@{}}
 \toprule()
 \begin{minipage}[b]{\linewidth}\raggedright
 \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
 1e-05
 \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
 0.0003162
 \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
 0.01
 \end{minipage} \\
 \midrule()
 \endhead
 natural & 0.820 \(+-\) 0.013 & 0.825 \(+-\) 0.005 & 0.788 \(+-\)
 0.019 \\
 hpf & 0.836 \(+-\) 0.008 & 0.825 \(+-\) 0.009 & 0.791
 \(+-\) 0.011 \\
 \bottomrule()\caption{Validation accuracies for VGG (ImageNette, low cutoff), variable
 decay}
 \end{longtable}
 
 \begin{longtable}[]{@{}
   >{\raggedright\arraybackslash}p{(\columnwidth - 6\tabcolsep) * \real{0.2703}}
   >{\raggedright\arraybackslash}p{(\columnwidth - 6\tabcolsep) * \real{0.2432}}
   >{\raggedright\arraybackslash}p{(\columnwidth - 6\tabcolsep) * \real{0.2432}}
   >{\raggedright\arraybackslash}p{(\columnwidth - 6\tabcolsep) * \real{0.2432}}@{}}
 \toprule()
 \begin{minipage}[b]{\linewidth}\raggedright
 \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
 1e-05
 \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
 0.0003162
 \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
 0.01
 \end{minipage} \\
 \midrule()
 \endhead
 natural & 0.820 \(+-\) 0.013 & 0.825 \(+-\) 0.005 & 0.788 \(+-\)
 0.019 \\
 hpf & 0.791 \(+-\) 0.013 & 0.789 \(+-\) 0.010 & 0.748
 \(+-\) 0.017 \\
 \bottomrule()\caption{Validation accuracies for VGG (ImageNette, high cutoff), variable
 decay}
 \end{longtable}
 
 \begin{longtable}[]{@{}
   >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.2174}}
   >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.1957}}
   >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.1957}}
   >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.1957}}
   >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.1957}}@{}}
 \toprule()
 \begin{minipage}[b]{\linewidth}\raggedright
 \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
 1
 \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
 2
 \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
 4
 \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
 8
 \end{minipage} \\
 \midrule()
 \endhead
 natural & 0.546 \(+-\) 0.006 & 0.612 \(+-\) 0.007 & 0.633 \(+-\) 0.005 &
 0.624 \(+-\) 0.006 \\
 hpf & 0.373 \(+-\) 0.019 & 0.404 \(+-\) 0.025 & 0.494
 \(+-\) 0.030 & 0.499 \(+-\) 0.097 \\
 \bottomrule()\caption{Validation accuracies for ConvActually, variable
 depth}
 \end{longtable}
 
 \begin{longtable}[]{@{}
   >{\raggedright\arraybackslash}p{(\columnwidth - 6\tabcolsep) * \real{0.2703}}
   >{\raggedright\arraybackslash}p{(\columnwidth - 6\tabcolsep) * \real{0.2432}}
   >{\raggedright\arraybackslash}p{(\columnwidth - 6\tabcolsep) * \real{0.2432}}
   >{\raggedright\arraybackslash}p{(\columnwidth - 6\tabcolsep) * \real{0.2432}}@{}}
 \toprule()
 \begin{minipage}[b]{\linewidth}\raggedright
 \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
 9
 \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
 20
 \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
 56
 \end{minipage} \\
 \midrule()
 \endhead
 natural & 0.920 \(+-\) 0.003 & 0.899 \(+-\) 0.003 & 0.902 \(+-\)
 0.003 \\
 hpf & 0.845 \(+-\) 0.007 & 0.830 \(+-\) 0.002 & 0.833
 \(+-\) 0.005 \\
 \bottomrule()\caption{Validation accuracies for ResNet, variable depth}
 \end{longtable}
 
 
 \begin{longtable}[]{@{}
   >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.2174}}
   >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.1957}}
   >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.1957}}
   >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.1957}}
   >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.1957}}@{}}
 \toprule()
 \begin{minipage}[b]{\linewidth}\raggedright
 \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
 11
 \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
 13
 \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
 16
 \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
 19
 \end{minipage} \\
 \midrule()
 \endhead
 natural & 0.872 \(+-\) 0.002 & 0.886 \(+-\) 0.002 & 0.888 \(+-\) 0.003 &
 0.890 \(+-\) 0.003 \\
 hpf & 0.797 \(+-\) 0.004 & 0.809 \(+-\) 0.003 & 0.807
 \(+-\) 0.002 & 0.809 \(+-\) 0.003 \\
 \bottomrule()\caption{Validation accuracies for VGG (CIFAR), variable
 depth}
 \end{longtable}
 
 
 \begin{longtable}[]{@{}
   >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.2174}}
   >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.1957}}
   >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.1957}}
   >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.1957}}
   >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.1957}}@{}}
 \toprule()
 \begin{minipage}[b]{\linewidth}\raggedright
 \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
 11
 \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
 13
 \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
 16
 \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
 19
 \end{minipage} \\
 \midrule()
 \endhead
 natural & 0.832 \(+-\) 0.008 & 0.826 \(+-\) 0.012 & 0.841 \(+-\) 0.010 &
 0.855 \(+-\) 0.007 \\
 hpf & 0.834 \(+-\) 0.008 & 0.840 \(+-\) 0.011 & 0.835
 \(+-\) 0.008 & 0.841 \(+-\) 0.014 \\
 \bottomrule()\caption{Validation accuracies for VGG (ImageNette, low cutoff), variable
 depth}
 \end{longtable}
 
 \begin{longtable}[]{@{}
   >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.2174}}
   >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.1957}}
   >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.1957}}
   >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.1957}}
   >{\raggedright\arraybackslash}p{(\columnwidth - 8\tabcolsep) * \real{0.1957}}@{}}
 \toprule()
 \begin{minipage}[b]{\linewidth}\raggedright
 \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
 11
 \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
 13
 \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
 16
 \end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
 19
 \end{minipage} \\
 \midrule()
 \endhead
 natural & 0.832 \(+-\) 0.008 & 0.826 \(+-\) 0.012 & 0.841 \(+-\) 0.010 &
 0.855 \(+-\) 0.007 \\
 hpf & 0.794 \(+-\) 0.012 & 0.789 \(+-\) 0.006 & 0.801
 \(+-\) 0.008 & 0.823 \(+-\) 0.009 \\
 \bottomrule()\caption{Validation accuracies for VGG (ImageNette, high cutoff), variable
 depth.}
 \end{longtable}
